M-DocSum: Do LVLMs Genuinely Comprehend Interleaved Image-Text in Document Summarization?

We investigate a critical yet under-explored question in Large Vision-Language Models (LVLMs): Do LVLMs genuinely comprehend interleaved image-text in the document? Existing document understanding benchmarks often assess LVLMs using question-answer formats, which are information-sparse and difficult to guarantee the coverage of long-range dependencies. To address this issue, we introduce a novel and challenging Multimodal Document Summarization Benchmark (M-DocSum-Bench), which comprises 500 high-quality arXiv papers, along with interleaved multimodal summaries aligned with human preferences. M-DocSum-Bench is a reference-based generation task and necessitates the generation of interleaved image-text summaries using provided reference images, thereby simultaneously evaluating capabilities in understanding, reasoning, localization, and summarization within complex multimodal document scenarios. To facilitate this benchmark, we develop an automated framework to construct summaries and propose a fine-grained evaluation method called M-DocEval. Moreover, we further develop a robust summarization baseline, i.e., M-DocSum-7B, by progressive two-stage training with diverse instruction and preference data. The extensive results on our M-DocSum-Bench reveal that the leading LVLMs struggle to maintain coherence and accurately integrate information within long and interleaved contexts, often exhibiting confusion between similar images and a lack of robustness. Notably, M-DocSum-7B achieves state-of-the-art performance compared to larger and closed-source models (including GPT-4o, Gemini Pro, Claude-3.5-Sonnet and Qwen2.5-VL-72B, etc.), demonstrating the potential of LVLMs for improved interleaved image-text understanding. The code, data, and models are available at https://github.com/stepfun-ai/M-DocSum-Bench.

==> tabs/A_4_shuffle.tex <==
\begin{table*}[h]
\caption{Comparison with Image Score and Decline Rates}
\centering
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{lcc}
\toprule
Models                      & Original IS & Shuffled IS \\
\midrule
GPT-4o                   & 0.638          & 0.533           \\
Gemini-pro                 & 0.553          & 0.501           \\
Claude-3-5-sonnet & 0.589          & 0.512           \\
Qwen2.5-VL-72B             & 0.517          & 0.491           \\
Qwen2-vl-72B               & 0.485          & 0.399           \\
Qwen2.5-vl-7B               & 0.423          & 0.373           \\
Qwen2-vl-7B                & 0.421          & 0.302           \\
Stage-1       & 0.615          & 0.450           \\
M-DocSum-7B      & 0.636          & 0.483           \\
M-DocSum-7B w/o stage-1                 & 0.556          & 0.405         \\
\bottomrule
\end{tabular}
}
\label{tab:shuffle}
\end{table*}


==> tabs/A_5_abstract.tex <==
\begin{table*}[h]
\caption{Comparison with Text Score and Decline Rates}
\centering
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{lcc}
\toprule
Models                     & Original TS & W/o abstract TS \\
\midrule
Qwen2.5-VL-7B                       & 0.517	&0.418           \\
Qwen2-VL-7B         &  0.449&	0.402           \\
InternVL2-8B & 0.513&	0.435          \\
InternVL2.5-8B             & 0.529&	0.488           \\
Stage-1                & 0.660&	0.605          \\
M-DocSum-7B               & 0.644&	0.615         \\

\bottomrule
\end{tabular}
}
\label{tab:abs}
\end{table*}

